VERITAS discovery of very high energy gamma-ray emission from S3 1227+25 and multiwavelength observations

We report the detection of very high energy gamma-ray emission from the blazar S3 1227+25 (VER J1230+253) with the Very Energetic Radiation Imaging Telescope Array System (VERITAS). VERITAS observations of the source were triggered by the detection of a hard-spectrum GeV flare on May 15, 2015 with the Fermi-Large Area Telescope (LAT). A combined five-hour VERITAS exposure on May 16th and May 18th resulted in a strong 13$\sigma$ detection with a differential photon spectral index, $\Gamma$ = 3.8 $\pm$ 0.4, and a flux level at 9% of the Crab Nebula above 120 GeV. This also triggered target of opportunity observations with Swift, optical photometry, polarimetry and radio measurements, also presented in this work, in addition to the VERITAS and Fermi-LAT data. A temporal analysis of the gamma-ray flux during this period finds evidence of a shortest variability timescale of $\tau_{obs}$ = 6.2 $\pm$ 0.9 hours, indicating emission from compact regions within the jet, and the combined gamma-ray spectrum shows no strong evidence of a spectral cut-off. An investigation into correlations between the multiwavelength observations found evidence of optical and gamma-ray correlations, suggesting a single-zone model of emission. Finally, the multiwavelength spectral energy distribution is well described by a simple one-zone leptonic synchrotron self-Compton radiation model.

==> ack.tex <==
\acknowledgments
\section*{Acknowledgements}

This research is supported by grants from the U.S. Department of Energy Office of Science, the U.S. National Science Foundation and the Smithsonian Institution, by NSERC in Canada, and by the Helmholtz Association in Germany. This research used resources provided by the Open Science Grid, which is supported by the National Science Foundation and the U.S. Department of Energy's Office of Science, and resources of the National Energy Research Scientific Computing Center (NERSC), a U.S. Department of Energy Office of Science User Facility operated under Contract No. DE-AC02-05CH11231. We acknowledge the excellent work of the technical support staff at the Fred Lawrence Whipple Observatory and at the collaborating institutions in the construction and operation of the instrument.

%VERITAS is supported by grants from the U.S. Department of Energy Office of Science, the U.S. National Science Foundation and the Smithsonian Institution, and by NSERC in Canada. We acknowledge the excellent work of the technical support staff at the Fred Lawrence Whipple Observatory and at the collaborating institutions in the construction and operation of the instrument. The VERITAS Collaboration is grateful to Trevor Weekes for his seminal contributions and leadership in the field of VHE gamma-ray astrophysics, and for his interest in the wider applications of IACTs, which made this study possible. Research at Lick Observatory is partially supported by  a generous gift from Google.


This work has made use of data from the Asteroid Terrestrial-impact Last Alert System (ATLAS) project. The Asteroid Terrestrial-impact Last Alert System
(ATLAS) project is primarily funded to search for near earth asteroids through NASA grants NN12AR55G, 80NSSC18K0284, and 80NSSC18K1575; byproducts of the NEO search include images and catalogs from the survey area. This work was
partially funded by Kepler/K2 grant J1944/80NSSC19K0112 and HST GO-15889, and STFC grants ST/T000198/1 and ST/S006109/1. The ATLAS science products have been made possible through the contributions of the University of Hawaii
Institute for Astronomy, the Queen’s University Belfast, the Space Telescope Science Institute, the South African Astronomical Observatory, and The Millennium Institute of Astrophysics (MAS), Chile.

==> authorlist.tex <==
\author{
A.~Acharyya\altaffilmark{0},
A.~Archer\altaffilmark{1},
W.~Benbow\altaffilmark{2},
R.~Bird\altaffilmark{3},
M.~Buchovecky\altaffilmark{4},
J.~H.~Buckley\altaffilmark{1},
V.~Bugaev\altaffilmark{1},
K.~Byrum\altaffilmark{5},
J.~V~Cardenzana\altaffilmark{6},
M.~Cerruti\altaffilmark{2},
X.~Chen\altaffilmark{7,8},
L.~Ciupik\altaffilmark{9},
E.~Collins-Hughes\altaffilmark{3},
M.~P.~Connolly\altaffilmark{10},
J.~D.~Eisch\altaffilmark{6},
A.~Falcone\altaffilmark{11},
Q.~Feng\altaffilmark{12},
J.~P.~Finley\altaffilmark{12},
H.~Fleischhack\altaffilmark{8},
A.~Flinders\altaffilmark{13},
L.~Fortson\altaffilmark{14},
A.~Furniss\altaffilmark{15},
G.~H.~Gillanders\altaffilmark{10},
S.~Griffin\altaffilmark{16},
J.~Grube\altaffilmark{9},
G.~Gyuk\altaffilmark{9},
N.~H{\aa}kansson\altaffilmark{7},
D.~Hanna\altaffilmark{16},
J.~Holder\altaffilmark{17},
T.~B.~Humensky\altaffilmark{18},
M.~H{\"u}tten\altaffilmark{8},
C.~A.~Johnson\altaffilmark{19},
P.~Kaaret\altaffilmark{20},
P.~Kar\altaffilmark{13},
N.~Kelley-Hoskins\altaffilmark{8},
M.~Kertzman\altaffilmark{21},
D.~Kieda\altaffilmark{13},
M.~Krause\altaffilmark{8},
F.~Krennrich\altaffilmark{6},
S.~Kumar\altaffilmark{17},
M.~J.~Lang\altaffilmark{10},
S.~McArthur\altaffilmark{12},
A.~McCann\altaffilmark{16},
K.~Meagher\altaffilmark{22},
J.~Millis\altaffilmark{23,23},
P.~Moriarty\altaffilmark{10},
R.~Mukherjee\altaffilmark{24},
D.~Nieto\altaffilmark{18},
R.~A.~Ong\altaffilmark{4},
N.~Park\altaffilmark{25},
V.~Pelassa\altaffilmark{2},
M.~Pohl\altaffilmark{7,8},
A.~Popkow\altaffilmark{4},
E.~Pueschel\altaffilmark{3},
J.~Quinn\altaffilmark{3},
K.~Ragan\altaffilmark{16},
G.~Ratliff\altaffilmark{9},
P.~T.~Reynolds\altaffilmark{26},
G.~T.~Richards\altaffilmark{22},
E.~Roache\altaffilmark{2},
J.~Rousselle\altaffilmark{4},
M.~Santander\altaffilmark{24},
G.~H.~Sembroski\altaffilmark{12},
K.~Shahinyan\altaffilmark{14},
A.~W.~Smith\altaffilmark{27},
D.~Staszak\altaffilmark{16},
I.~Telezhinsky\altaffilmark{7,8},
J.~V.~Tucci\altaffilmark{12},
J.~Tyler\altaffilmark{16},
V.~V.~Vassiliev\altaffilmark{4},
S.~P.~Wakely\altaffilmark{25},
O.~M.~Weiner\altaffilmark{18},
A.~Weinstein\altaffilmark{6},
A.~Wilhelm\altaffilmark{7,8},
D.~A.~Williams\altaffilmark{19},
B.~Zitzer\altaffilmark{5}
}

\altaffiltext{1}{Department of Physics, Washington University, St. Louis, MO 63130, USA}
\altaffiltext{2}{Fred Lawrence Whipple Observatory, Harvard-Smithsonian Center for Astrophysics, Amado, AZ 85645, USA}
\altaffiltext{3}{School of Physics, University College Dublin, Belfield, Dublin 4, Ireland}
\altaffiltext{4}{Department of Physics and Astronomy, University of California, Los Angeles, CA 90095, USA}
\altaffiltext{5}{Argonne National Laboratory, 9700 S. Cass Avenue, Argonne, IL 60439, USA}
\altaffiltext{6}{Department of Physics and Astronomy, Iowa State University, Ames, IA 50011, USA}
\altaffiltext{7}{Institute of Physics and Astronomy, University of Potsdam, 14476 Potsdam-Golm, Germany}
\altaffiltext{8}{DESY, Platanenallee 6, 15738 Zeuthen, Germany}
\altaffiltext{9}{Astronomy Department, Adler Planetarium and Astronomy Museum, Chicago, IL 60605, USA}
\altaffiltext{10}{School of Physics, National University of Ireland Galway, University Road, Galway, Ireland}
\altaffiltext{11}{Department of Astronomy and Astrophysics, 525 Davey Lab, Pennsylvania State University, University Park, PA 16802, USA}
\altaffiltext{12}{Department of Physics and Astronomy, Purdue University, West Lafayette, IN 47907, USA}
\altaffiltext{13}{Department of Physics and Astronomy, University of Utah, Salt Lake City, UT 84112, USA}
\altaffiltext{14}{School of Physics and Astronomy, University of Minnesota, Minneapolis, MN 55455, USA}
\altaffiltext{15}{Department of Physics, California State University - East Bay, Hayward, CA 94542, USA}
\altaffiltext{16}{Physics Department, McGill University, Montreal, QC H3A 2T8, Canada}
\altaffiltext{17}{Department of Physics and Astronomy and the Bartol Research Institute, University of Delaware, Newark, DE 19716, USA} 
\altaffiltext{18}{Physics Department, Columbia University, New York, NY 10027, USA}
\altaffiltext{19}{Santa Cruz Institute for Particle Physics and Department of Physics, University of California, Santa Cruz, CA 95064, USA}
\altaffiltext{20}{Department of Physics and Astronomy, University of Iowa, Van Allen Hall, Iowa City, IA 52242, USA}
\altaffiltext{21}{Department of Physics and Astronomy, DePauw University, Greencastle, IN 46135-0037, USA}
\altaffiltext{22}{School of Physics and Center for Relativistic Astrophysics, Georgia Institute of Technology, 837 State Street NW, Atlanta, GA 30332-0430}
\altaffiltext{23}{Department of Physics, Anderson University, 1100 East 5th Street, Anderson, IN 46012}
\altaffiltext{24}{Department of Physics and Astronomy, Barnard College, Columbia University, NY 10027, USA}
\altaffiltext{25}{Enrico Fermi Institute, University of Chicago, Chicago, IL 60637, USA}
\altaffiltext{26}{Department of Applied Science, Cork Institute of Technology, Bishopstown, Cork, Ireland}
\altaffiltext{27}{University of Maryland, College Park / NASA GSFC, College Park, MD 20742, USA}

==> authors.tex <==
\author[0000-0002-2028-9230]{A.~Acharyya}\affiliation{Department of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA}
\author[0000-0002-9021-6192]{C.~B.~Adams}\affiliation{Physics Department, Columbia University, New York, NY 10027, USA}
\author{A.~Archer}\affiliation{Department of Physics and Astronomy, DePauw University, Greencastle, IN 46135-0037, USA}
\author[0000-0002-3886-3739]{P.~Bangale}\affiliation{Department of Physics and Astronomy and the Bartol Research Institute, University of Delaware, Newark, DE 19716, USA}
\author[0000-0003-2098-170X]{W.~Benbow}\affiliation{Center for Astrophysics $|$ Harvard \& Smithsonian, Cambridge, MA 02138, USA}
\author[0000-0002-6208-5244]{A.~Brill}\affiliation{N.A.S.A./Goddard Space-Flight Center, Code 661, Greenbelt, MD 20771, USA}
\author{J.~L.~Christiansen}\affiliation{Physics Department, California Polytechnic State University, San Luis Obispo, CA 94307, USA}
\author{A.~J.~Chromey}\affiliation{Center for Astrophysics $|$ Harvard \& Smithsonian, Cambridge, MA 02138, USA}
\author[0000-0002-1853-863X]{M.~Errando}\affiliation{Department of Physics, Washington University, St. Louis, MO 63130, USA}
\author[0000-0002-5068-7344]{A.~Falcone}\affiliation{Department of Astronomy and Astrophysics, 525 Davey Lab, Pennsylvania State University, University Park, PA 16802, USA}
\author[0000-0001-6674-4238]{Q.~Feng}\affiliation{Center for Astrophysics $|$ Harvard \& Smithsonian, Cambridge, MA 02138, USA}
\author{J.~P.~Finley}\affiliation{Department of Physics and Astronomy, Purdue University, West Lafayette, IN 47907, USA}
\author[0000-0002-2944-6060]{G.~M.~Foote}\affiliation{Department of Physics and Astronomy and the Bartol Research Institute, University of Delaware, Newark, DE 19716, USA}
\author[0000-0002-1067-8558]{L.~Fortson}\affiliation{School of Physics and Astronomy, University of Minnesota, Minneapolis, MN 55455, USA}
\author[0000-0003-1614-1273]{A.~Furniss}\affiliation{Department of Physics, California State University - East Bay, Hayward, CA 94542, USA}
\author{G.~Gallagher}\affiliation{Department of Physics and Astronomy, Ball State University, Muncie, IN 47306, USA}
\author[0000-0002-0109-4737]{W.~Hanlon}\affiliation{Center for Astrophysics $|$ Harvard \& Smithsonian, Cambridge, MA 02138, USA}
\author[0000-0002-8513-5603]{D.~Hanna}\affiliation{Physics Department, McGill University, Montreal, QC H3A 2T8, Canada}
\author[0000-0003-3878-1677]{O.~Hervet}\affiliation{Santa Cruz Institute for Particle Physics and Department of Physics, University of California, Santa Cruz, CA 95064, USA}
\author[0000-0001-6951-2299]{C.~E.~Hinrichs}\affiliation{Center for Astrophysics $|$ Harvard \& Smithsonian, Cambridge, MA 02138, USA and Department of Physics and Astronomy, Dartmouth College, 6127 Wilder Laboratory, Hanover, NH 03755 USA}
\author{J.~Hoang}\affiliation{Santa Cruz Institute for Particle Physics and Department of Physics, University of California, Santa Cruz, CA 95064, USA}
\author[0000-0002-6833-0474]{J.~Holder}\affiliation{Department of Physics and Astronomy and the Bartol Research Institute, University of Delaware, Newark, DE 19716, USA}
\author[0000-0002-1089-1754]{W.~Jin}\affiliation{Department of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA}
\author[0009-0008-2688-0815]{M.~N.~Johnson}\affiliation{Santa Cruz Institute for Particle Physics and Department of Physics, University of California, Santa Cruz, CA 95064, USA}
\author[0000-0002-3638-0637]{P.~Kaaret}\affiliation{Department of Physics and Astronomy, University of Iowa, Van Allen Hall, Iowa City, IA 52242, USA}
\author{M.~Kertzman}\affiliation{Department of Physics and Astronomy, DePauw University, Greencastle, IN 46135-0037, USA}
\author[0000-0003-4785-0101]{D.~Kieda}\affiliation{Department of Physics and Astronomy, University of Utah, Salt Lake City, UT 84112, USA}
\author[0000-0002-4260-9186]{T.~K.~Kleiner}\affiliation{DESY, Platanenallee 6, 15738 Zeuthen, Germany}
\author[0000-0002-4289-7106]{N.~Korzoun}\affiliation{Department of Physics and Astronomy and the Bartol Research Institute, University of Delaware, Newark, DE 19716, USA}
\author{F.~Krennrich}\affiliation{Department of Physics and Astronomy, Iowa State University, Ames, IA 50011, USA}
\author[0000-0003-4641-4201]{M.~J.~Lang}\affiliation{School of Natural Sciences, University of Galway, University Road, Galway, H91 TK33, Ireland}
\author[0000-0003-3802-1619]{M.~Lundy}\affiliation{Physics Department, McGill University, Montreal, QC H3A 2T8, Canada}
\author[0000-0001-9868-4700]{G.~Maier}\affiliation{DESY, Platanenallee 6, 15738 Zeuthen, Germany}
\author{C.~E~McGrath}\affiliation{School of Physics, University College Dublin, Belfield, Dublin 4, Ireland}
\author[0000-0001-7106-8502]{M.~J.~Millard}\affiliation{Department of Physics and Astronomy, University of Iowa, Van Allen Hall, Iowa City, IA 52242, USA}
\author{J.~Millis}\affiliation{Department of Physics and Astronomy, Ball State University, Muncie, IN 47306, USA and Department of Physics, Anderson University, 1100 East 5th Street, Anderson, IN 46012}
\author[0000-0001-5937-446X]{C.~L.~Mooney}\affiliation{Department of Physics and Astronomy and the Bartol Research Institute, University of Delaware, Newark, DE 19716, USA}
\author[0000-0002-1499-2667]{P.~Moriarty}\affiliation{School of Natural Sciences, University of Galway, University Road, Galway, H91 TK33, Ireland}
\author[0000-0002-3223-0754]{R.~Mukherjee}\affiliation{Department of Physics and Astronomy, Barnard College, Columbia University, NY 10027, USA}
\author[0000-0002-9296-2981]{S.~O'Brien}\affiliation{Physics Department, McGill University, Montreal, QC H3A 2T8, Canada}
\author[0000-0002-4837-5253]{R.~A.~Ong}\affiliation{Department of Physics and Astronomy, University of California, Los Angeles, CA 90095, USA}
\author[0000-0001-7861-1707]{M.~Pohl}\affiliation{Institute of Physics and Astronomy, University of Potsdam, 14476 Potsdam-Golm, Germany and DESY, Platanenallee 6, 15738 Zeuthen, Germany}
\author[0000-0002-0529-1973]{E.~Pueschel}\affiliation{DESY, Platanenallee 6, 15738 Zeuthen, Germany}
\author[0000-0002-4855-2694]{J.~Quinn}\affiliation{School of Physics, University College Dublin, Belfield, Dublin 4, Ireland}
\author[0000-0002-5351-3323]{K.~Ragan}\affiliation{Physics Department, McGill University, Montreal, QC H3A 2T8, Canada}
\author{P.~T.~Reynolds}\affiliation{Department of Physical Sciences, Munster Technological University, Bishopstown, Cork, T12 P928, Ireland}
\author[0000-0002-7523-7366]{D.~Ribeiro}\affiliation{School of Physics and Astronomy, University of Minnesota, Minneapolis, MN 55455, USA}
\author{E.~Roache}\affiliation{Center for Astrophysics $|$ Harvard \& Smithsonian, Cambridge, MA 02138, USA}
\author[0000-0003-1387-8915]{I.~Sadeh}\affiliation{DESY, Platanenallee 6, 15738 Zeuthen, Germany}
\author{A.~C.~Sadun}\affiliation{Department of Physics, University of Colorado Denver, Campus Box 157, P.O.Box 173364, Denver CO 80217, USA}
\author[0000-0002-3171-5039]{L.~Saha}\affiliation{Center for Astrophysics $|$ Harvard \& Smithsonian, Cambridge, MA 02138, USA}
\author{M.~Santander}\affiliation{Department of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA}
\author{G.~H.~Sembroski}\affiliation{Department of Physics and Astronomy, Purdue University, West Lafayette, IN 47907, USA}
\author[0000-0002-9856-989X]{R.~Shang}\affiliation{Department of Physics and Astronomy, Barnard College, Columbia University, NY 10027, USA}
\author[0000-0003-3407-9936]{M.~Splettstoesser}\affiliation{Santa Cruz Institute for Particle Physics and Department of Physics, University of California, Santa Cruz, CA 95064, USA}
\author{A.~Kaushik~Talluri}\affiliation{School of Physics and Astronomy, University of Minnesota, Minneapolis, MN 55455, USA}
\author{J.~V.~Tucci}\affiliation{Department of Physics, Indiana University-Purdue University Indianapolis, Indianapolis, IN 46202, USA}
\author{V.~V.~Vassiliev}\affiliation{Department of Physics and Astronomy, University of California, Los Angeles, CA 90095, USA}
\author[0000-0003-2740-9714]{D.~A.~Williams}\affiliation{Santa Cruz Institute for Particle Physics and Department of Physics, University of California, Santa Cruz, CA 95064, USA}
\author[0000-0002-2730-2733]{S.~L.~Wong}\affiliation{Physics Department, McGill University, Montreal, QC H3A 2T8, Canada}
\author[0000-0002-2024-8199]{Talvikki Hovatta}\affiliation{Finnish Centre for Astronomy with ESO (FINCA), University of Turku, FI-20014, Turku, Finland}  \affiliation{Aalto University Mets\"ahovi Radio Observatory, Mets\"ahovintie 114,02540 Kylm\"al\"a, Finland}
\author[0000-0001-6158-1708]{Svetlana G. Jorstad}\affiliation{Institute for Astrophysical Research, Boston University, 725 Commonwealth Avenue, Boston, MA 02215, USA}
\author[0000-0001-6314-9177]{Sebastian Kiehlmann} \affiliation{Institute of Astrophysics, Foundation for Research and Technology-Hellas, GR-71110 Heraklion, Greece} \affiliation{Department of Physics, Univ. of Crete, GR-70013 Heraklion, Greece}
\author[0000-0002-0393-0647]{Anne L\"ahteenm\"aki}\affiliation{Aalto University Mets\"ahovi Radio Observatory, Mets\"ahovintie 114,02540 Kylm\"al\"a, Finland} \affiliation{Aalto University Department of Electronics and Nanoengineering, P.O. BOX 15500, FI-00076 AALTO, Finland} 
\author[0000-0001-9200-4006]{Ioannis Liodakis} \affiliation{Finnish Center for Astronomy with ESO, University of Turku, FI-20014, Finland}
\author[0000-0001-7396-3332]{Alan P. Marscher}\affiliation{Institute for Astrophysical Research, Boston University, 725 Commonwealth Avenue, Boston, MA 02215, USA}
\author[0000-0002-5491-5244]{Walter Max-Moerbeck} \affiliation{Departamento de Astronom\'ia, Universidad de Chile, Camino El Observatorio 1515, Las Condes, Santiago, Chile}
\author[0000-0001-9152-961X]{Anthony C. S. Readhead} \affiliation{Owens Valley Radio Observatory, California Institute of Technology, Pasadena, CA 91125, USA}
\author[0000-0001-5704-271X]{Rodrigo Reeves} \affiliation{Departamento de Astronom\'a, Universidad de Concepti\'on, Concepci\'on, Chile}
\author[0000-0002-5083-3663]{Paul S. Smith}\affiliation{Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA}
\author[0000-0003-1249-6026]{Merja Tornikoski}\affiliation{Aalto University Mets\"ahovi Radio Observatory, Mets\"ahovintie 114,02540 Kylm\"al\"a, Finland}

==> vhe_photons.tex <==
The \textit{Fermi} tool \textit{gtobssim} can be used to simulate \textit{Fermi}-LAT observations of S3 1227+25, taking into account IRFs and the spacecraft pointing history. 
The simulations assume a range of cut-off energies and the energy distribution of the simulated photons, when compared to the energy  of the observed photons, should reveal if the GeV photon emission is compatible with the cut-off energy predicted. Attenuation due to the EBL is also accounted for using the opacities, $\tau$, stated in the \cite{RN10} model to calculate the likely attenuation. 

The intrinsic absorption is accounted for by choosing a number of cut-off energies, ${E}_{\text{cut}}$, evenly spaced in the interval 90--180 GeV, based on the result $E_{\text{cut}} = 142 \pm 43$~GeV obtained from the joint fit to the combined gamma-ray spectrum. The resultant differential flux used for simulations is given by:

\begin{equation}
% \hspace*{2cm}
  \centering
   \frac{dN}{dE}=N_{0} \left(\frac{E}{E_0}\right)^{-\gamma}  e^{-\left(\frac{E}{E_{\text{cut}}}\right)} e^{-\tau}
	\label{eq:10}
\end{equation}

where once again ${E_0}$ is the pivot energy in MeV, $N_{0}$ is the normalisation in units of photons $\text{cm}^{-2}\text{s}^{-1} \text{MeV}^{-1}$ and $\gamma$ the spectral index. 

The energy distribution of the most energetic photons simulated, determined using 1000 simulations with different seed variables at each cut-off energy, seen in Fig.~\ref{fig:Fig7}, shows the 1$\sigma$, 2$\sigma$ and 3$\sigma$ confidence intervals as a function of the different cut-off energies used in the simulations. For comparison, the energy of most energetic photon observed with the \textit{Fermi}-LAT during the period investigated is shown along with its corresponding uncertainty. 

The results indicate that the cut-off energy range predicted from the joint fit to the gamma-ray spectrum is compatible with the most energetic GeV photon observed with the \textit{Fermi}-LAT during this period. In conjunction with the GeV photons which coincide with the VERITAS detection, this could potentially imply a common origin. 
Furthermore, the expected onset of intrinsic cut-off due to interaction with Lyman alpha photons in the BLR is $E_{\text{Ly}\alpha}=\frac{25}{1+z}$ GeV for a source at redshift $z$ (\cite{RN3}) and would be $E_{\text{Ly}\alpha}=22.03$~GeV for S3 1227+25. This is not compatible with both the energy cut-off range predicted from the joint fit to the gamma-ray spectrum and the GeV photons observed and can be interpreted as evidence that the VHE photon emission is constrained to within the MT, at parsec scale distances from the central engine.

\begin{figure}
    \centering
    \resizebox{0.5 \textwidth}{!}{
    \includegraphics{fig/results.pdf}}
    \caption{The energy distributions of the most energetic photons, $E_{{\gamma}}$, obtained from Monte Carlo simulations as a function of the cut-off energy, $E_{\text{cut}}$, used in the simulations (see equation \ref{eq:10}) for S3 1227+25. The shaded regions represent the 1$\sigma$, 2$\sigma$ and 3$\sigma$ confidence intervals from darker to lighter shades respectively. The green dashed line is the energy of most energetic photon observed with the \textit{Fermi}-LAT during the period corresponding to the VERITAS detection along with the corresponding uncertainty.}
    \label{fig:Fig7}
\end{figure}

